Groupwise Query Performance Prediction with BERT

While large-scale pre-trained language models like BERT have advanced the state-of-the-art in IR, its application in query performance prediction (QPP) is so far based on pointwise modeling of individual queries. Meanwhile, recent studies suggest that the cross-attention modeling of a group of documents can effectively boost performances for both learning-to-rank algorithms and BERT-based re-ranking. To this end, a BERT-based groupwise QPP model is proposed, in which the ranking contexts of a list of queries are jointly modeled to predict the relative performance of individual queries. Extensive experiments on three standard TREC collections showcase effectiveness of our approach. Our code is available at https://github.com/VerdureChen/Group-QPP.

==> TABLES.tex <==
\begin{table}[]
\centering
\caption{Polit Study on BERT-Base.}
\label{tab:Polit}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l|l|llllll}
\hline
\multirow{3}{*}{Training Label} &  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Doc/Q for \\ Training\end{tabular}} & \multicolumn{6}{c}{Target Metric: AP@1000} \\ \cline{3-8} 
                       &      & \multicolumn{2}{l}{Robust04}    & \multicolumn{2}{l}{GOV2}        & \multicolumn{2}{l}{ClueWeb09-B} \\ \cline{3-8} 
                       &      & P-$\rho$       & K-$\tau$       & P-$\rho$       & K-$\tau$     & P-$\rho$       & K-$\tau$             \\ \hline
\multirow{2}{*}{P@k}   & 1000 & 0.559          & 0.401          & \textbf{0.645} & \textbf{0.475} & 0.350          & 0.233          \\ \cline{2-2}
                       & 100  & \textbf{0.585} & \textbf{0.423} & 0.637          & 0.454          & 0.393          & 0.271          \\ \cline{1-2}
\multirow{2}{*}{AP@1k} & 1000 & 0.346          & 0.231          & 0.151          & 0.081          & \textbf{0.476} & \textbf{0.345} \\ \cline{2-2}
                       & 100  & 0.520          & 0.360          & 0.505          & 0.345          & 0.447          & 0.321          \\ \hline
\end{tabular}%
}
\end{table}


\begin{table*}[!ht]
\centering
\caption{Effectiveness of groupwise model. For BERT-based models, we use P@k for Robust04 and GOV2, AP@1k for ClueWeb09-B as the training labels.}
\label{tab:effectiveness}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|llllll|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{Target Metric: AP@1000}                                                         \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & \multicolumn{2}{l}{Robust04} & \multicolumn{2}{l}{GOV2} & \multicolumn{2}{l|}{ClueWeb09-B} \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                        & P-$\rho$       & K-$\tau$       & P-$\rho$       & K-$\tau$     & P-$\rho$       & K-$\tau$      \\ \hline
Clarity                                       & 0.528          & 0.385          & 0.428          & 0.291          & 0.300          & 0.213        \\
QF                                            & 0.390          & 0.324          & 0.447          & 0.314          & 0.163          & 0.072          \\
WIG                                           & 0.546          & 0.379          & 0.502          & 0.346          & 0.316          & 0.210          \\
NQC                                           & 0.516          & 0.388          & 0.381          & 0.323          & 0.127          & 0.138          \\
SMV                                           & 0.534          & 0.378          & 0.352          & 0.303          & 0.236          & 0.183          \\
UEF                                           & 0.502          & 0.402          & 0.470          & 0.329          & 0.301          & 0.211          \\
$\sigma_{k}$                                  & 0.522          & 0.389          & 0.381          & 0.323          & 0.234          & 0.177          \\
$n(\sigma_{X\%})$                            & 0.589          & 0.386          & 0.556          & 0.386          & 0.334          & {\ul 0.247}   \\
RSD                                           & 0.455          & 0.352          & 0.444          & 0.276          & 0.193          & 0.096          \\
WAND[$n(\sigma_{X\%})$]                      & 0.566          & 0.386          & {\ul 0.580}  &{\ul 0.411}  & 0.236         & 0.142          \\
NeuralQPP                                    & {\ul0.611} & {\ul 0.408}  & 0.540          & 0.357          & {\ul 0.367}  & 0.229          \\\hline
\multicolumn{7}{|l|}{BERT-Baselines}                        \\ \hline
BERT-Small                            & 0.591          & 0.391          & 0.615          & 0.436          & 0.394          & 0.278          \\
BERT-Base                             & 0.585          & 0.423          & 0.637          & 0.454          & 0.447          & 0.321 \\
BERT-Large                            & 0.579         &  0.422          & 0.645          &  0.461          & 0.342           &  0.251       \\ \hline
% \multicolumn{7}{|l|}{BERT-Base }                                                                                                                    \\ \hline
% (P@k\_1000)                                & 0.559          & 0.401          & \textbf{0.645}    & \textbf{0.475}  & 0.350          & 0.233          \\
% (AP@1k\_1000)                              & 0.346          & 0.231          & 0.151          & 0.081        & \textbf{0.476}    & \textbf{0.345}          \\
% (P@k\_100)                                 & \textbf{0.585}   & \textbf{0.423}     & 0.637    & 0.454          & 0.393          & 0.271          \\
% (AP@1k\_100)                               & 0.520          & 0.360          & 0.505          & 0.345          & 0.447          & 0.321          \\ \hline
\multicolumn{7}{|l|}{BERT-Small+Groupwise}                        \\ \hline
(R+Q+D)                      & 0.590          & 0.419          & 0.680          & 0.500          & 0.437          & 0.305         \\
% (Random\_100\_Small)                            &                &                &                &                & 0.443          & 0.306          \\ 
\hline
\multicolumn{7}{|l|}{BERT-Base+Groupwise   }                     \\  \hline
(Random order)                            & 0.608          & 0.449          & 0.665          & 0.479          & {\ul 0.481} & {\ul 0.353} \\
                                        % 
(Query order)                             & \textbf{0.615} & 0.456          & 0.676          & 0.486          & 0.455          &  0.327          \\
(Doc order)                               & 0.563          & 0.383          & 0.660          & 0.476          & 0.365          &  0.262         \\
(Query+Doc)                               & 0.598          & 0.452          & {\ul 0.682} & {\ul 0.496} & 0.438          &  0.317         \\
(R+Q+D)                                   & 0.608          & {\ul 0.460} & 0.676          & 0.489          & 0.469          & 0.342          \\ \hline
\multicolumn{7}{|l|}{BERT-Large+Groupwise}                        \\  \hline
(R+Q+D)                             & 0.612          & \textbf{0.470} & \textbf{0.688} & \textbf{0.508} & \textbf{0.545} &\textbf{0.399}    \\
% (Random\_100\_Large)                   &                &                &                &                & 0.531        &  0.396        \\ 
\hline

\end{tabular} 
}
\end{table*}


% \begin{table*}[!t]
% \centering
% \caption{Effectiveness of groupwise model. For model with groupwise scorer, we use P@k for Robust04 and GOV2, AP@1k for ClueWeb09-B as the training labels.}
% \label{tab:effectiveness}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{|l|llllll|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{Target Metric: AP@1000}                                                         \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{2}{l}{Robust04} & \multicolumn{2}{l}{GOV2} & \multicolumn{2}{l|}{ClueWeb09-B} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                        & P-$\rho$       & K-$\tau$       & P-$\rho$       & K-$\tau$     & P-$\rho$       & K-$\tau$      \\ \hline
% Clarity                                       & 0.528          & 0.385          & 0.428          & 0.291          & 0.300          & 0.213        \\
% QF                                            & 0.390          & 0.324          & 0.447          & 0.314          & 0.163          & 0.072          \\
% WIG                                           & 0.546          & 0.379          & 0.502          & 0.346          & 0.316          & 0.210          \\
% NQC                                           & 0.516          & 0.388          & 0.381          & 0.323          & 0.127          & 0.138          \\
% SMV                                           & 0.534          & 0.378          & 0.352          & 0.303          & 0.236          & 0.183          \\
% UEF                                           & 0.502          & 0.402          & 0.470          & 0.329          & 0.301          & 0.211          \\
% $\sigma_{k}$                                  & 0.522          & 0.389          & 0.381          & 0.323          & 0.234          & 0.177          \\
% $n(\sigma_{X\%})$                            & 0.589          & 0.386          & 0.556          & 0.386          & 0.334          & {\ul 0.247}   \\
% RSD                                           & 0.455          & 0.352          & 0.444          & 0.276          & 0.193          & 0.096          \\
% WAND[$n(\sigma_{X\%})$]                      & 0.566          & 0.386          & {\ul 0.580}  &{\ul 0.411}  & 0.236         & 0.142          \\
% NeuralQPP                                    & {\ul0.611} & {\ul 0.408}  & 0.540          & 0.357          & {\ul 0.367}  & 0.229          \\\hline
% \multicolumn{7}{|l|}{BERT-Baselines}                        \\ \hline
% BERT-Small                            & 0.591          & 0.391          & 0.615          & 0.436          & 0.394          & 0.278          \\
% BERT-Base                             & 0.585          & 0.423          & 0.637          & 0.454          & 0.476          & 0.345 \\
% BERT-Large                            &                &                & 0.645          &  0.461          &                &            \\ \hline
% % \multicolumn{7}{|l|}{BERT-Base }                                                                                                                    \\ \hline
% % (P@k\_1000)                                & 0.559          & 0.401          & \textbf{0.645}    & \textbf{0.475}  & 0.350          & 0.233          \\
% % (AP@1k\_1000)                              & 0.346          & 0.231          & 0.151          & 0.081        & \textbf{0.476}    & \textbf{0.345}          \\
% % (P@k\_100)                                 & \textbf{0.585}   & \textbf{0.423}     & 0.637    & 0.454          & 0.393          & 0.271          \\
% % (AP@1k\_100)                               & 0.520          & 0.360          & 0.505          & 0.345          & 0.447          & 0.321          \\ \hline
% \multicolumn{7}{|l|}{BERT-Small+Groupwise}                        \\ \hline
% (R+Q+D)                      & 0.590          & 0.419          & 0.680          & 0.500          & 0.437          & 0.305         \\
% % (Random\_100\_Small)                            &                &                &                &                & 0.443          & 0.306          \\ 
% \hline
% \multicolumn{7}{|l|}{BERT-Base+Groupwise   }                     \\  \hline
% (Random order)                            & 0.608          & 0.449          & 0.665          & 0.479          & \textbf{0.481} & \textbf{0.353} \\
% (Query order)                             & \textbf{0.615} & 0.456          & 0.676          & 0.486          & 0.455          &  0.327          \\
% (Doc order)                               & 0.563          & 0.383          & 0.660          & 0.476          & 0.365          &  0.262         \\
% (Query+Doc)                               & 0.598          & 0.452          & \textbf{0.682} & \textbf{0.496} & 0.438          &  0.317         \\
% (R+Q+D)                                   & 0.608          & \textbf{0.460} & 0.676          & 0.489          & 0.447          & 0.323          \\ \hline
% \multicolumn{7}{|l|}{BERT-Large+Groupwise}                        \\  \hline
% (R+Q+D)                             & 0.612          & \textbf{0.470} & \textbf{0.688} & \textbf{0.508} & \textbf{0.545} &\textbf{0.399}    \\
% % (Random\_100\_Large)                   &                &                &                &                & 0.531        &  0.396        \\ 
% \hline

% \end{tabular} 
% }
% \end{table*}


% \begin{table*}[!t]
% \centering
% \caption{Effectiveness of groupwise model. For model with groupwise scorer, we use P@k for Robust04 and GOV2, AP@1k for ClueWeb09-B as the training labels.}
% \label{tab:effectiveness}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{|l|llllll|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{Target Metric: AP@1000}                                                         \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{2}{l}{Robust04} & \multicolumn{2}{l}{GOV2} & \multicolumn{2}{l|}{ClueWeb09-B} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                        & P-$\rho$       & K-$\tau$       & P-$\rho$       & K-$\tau$     & P-$\rho$       & K-$\tau$      \\ \hline
% Clarity                                       & 0.528          & 0.385          & 0.428          & 0.291          & 0.300          & 0.213        \\
% QF                                            & 0.390          & 0.324          & 0.447          & 0.314          & 0.163          & 0.072          \\
% WIG                                           & 0.546          & 0.379          & 0.502          & 0.346          & 0.316          & 0.210          \\
% NQC                                           & 0.516          & 0.388          & 0.381          & 0.323          & 0.127          & 0.138          \\
% SMV                                           & 0.534          & 0.378          & 0.352          & 0.303          & 0.236          & 0.183          \\
% UEF                                           & 0.502          & 0.402          & 0.470          & 0.329          & 0.301          & 0.211          \\
% $\sigma_{k}$                                  & 0.522          & 0.389          & 0.381          & 0.323          & 0.234          & 0.177          \\
% $n(\sigma_{X\%})$                            & 0.589          & 0.386          & 0.556          & 0.386          & 0.334          & {\ul 0.247}   \\
% RSD                                           & 0.455          & 0.352          & 0.444          & 0.276          & 0.193          & 0.096          \\
% WAND[$n(\sigma_{X\%})$]                      & 0.566          & 0.386          & {\ul 0.580}  &{\ul 0.411}  & 0.236         & 0.142          \\
% NeuralQPP                                    & {\ul0.611} & {\ul 0.408}  & 0.540          & 0.357          & {\ul 0.367}  & 0.229          \\\hline
% \multicolumn{7}{|l|}{BERT-Baselines}                        \\ \hline
% BERT-Small                            & 0.591          & 0.391          & 0.615          & 0.436          & 0.394          & 0.278          \\
% BERT-Base                             & 0.585          & 0.423          & 0.637          & 0.454          & 0.476          & 0.345 \\
% BERT-Large                            &                &                & 0.645          &  0.461          &                &            \\ \hline
% % \multicolumn{7}{|l|}{BERT-Base }                                                                                                                    \\ \hline
% % (P@k\_1000)                                & 0.559          & 0.401          & \textbf{0.645}    & \textbf{0.475}  & 0.350          & 0.233          \\
% % (AP@1k\_1000)                              & 0.346          & 0.231          & 0.151          & 0.081        & \textbf{0.476}    & \textbf{0.345}          \\
% % (P@k\_100)                                 & \textbf{0.585}   & \textbf{0.423}     & 0.637    & 0.454          & 0.393          & 0.271          \\
% % (AP@1k\_100)                               & 0.520          & 0.360          & 0.505          & 0.345          & 0.447          & 0.321          \\ \hline
% \multicolumn{7}{|l|}{BERT+Groupwise   }                     \\  \hline
% (Random order)-B                            & 0.608          & 0.449          & 0.665          & 0.479          & 0.481 & 0.353 \\
% (Query order)-B                             & \textbf{0.615} & 0.456          & 0.676          & 0.486          & 0.455          &  0.327          \\
% (Doc order)-B                               & 0.563          & 0.383          & 0.660          & 0.476          & 0.365          &  0.262         \\
% (Query+Doc)-B                               & 0.598          & 0.452          & 0.682   & 0.496 & 0.438          &  0.317         \\
% (R+Q+D)-S                      & 0.590          & 0.419          & 0.680          & 0.500          & 0.437          & 0.305         \\
% (R+Q+D)-B                                   & 0.608          & 0.460 & 0.676          & 0.489          & 0.447          & 0.323          \\ 
% (R+Q+D)-L                             & 0.612          & \textbf{0.470} & \textbf{0.688} & \textbf{0.508} & \textbf{0.545} &\textbf{0.399}    \\
% % (Random\_100\_Large)                   &                &                &                &                & 0.531        &  0.396        \\ 
% \hline

% \end{tabular} 
% }
% \end{table*}

% \begin{table*}[!t]
% \centering
% \caption{Effectiveness of groupwise model. For model with groupwise scorer, we use P@k for Robust04 and GOV2, AP@1k for ClueWeb09-B as the training labels.}
% \label{tab:effectiveness}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{|l|llllll|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{Target Metric: AP@1000}                                                         \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{2}{l}{Robust04} & \multicolumn{2}{l}{GOV2} & \multicolumn{2}{l|}{ClueWeb09-B} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                        & P-$\rho$       & K-$\tau$       & P-$\rho$       & K-$\tau$     & P-$\rho$       & K-$\tau$      \\ \hline
% Clarity                                       & 0.528          & 0.385          & 0.428          & 0.291          & 0.300          & 0.213        \\
% QF                                            & 0.390          & 0.324          & 0.447          & 0.314          & 0.163          & 0.072          \\
% WIG                                           & 0.546          & 0.379          & 0.502          & 0.346          & 0.316          & 0.210          \\
% NQC                                           & 0.516          & 0.388          & 0.381          & 0.323          & 0.127          & 0.138          \\
% SMV                                           & 0.534          & 0.378          & 0.352          & 0.303          & 0.236          & 0.183          \\
% UEF                                           & 0.502          & 0.402          & 0.470          & 0.329          & 0.301          & 0.211          \\
% $\sigma_{k}$                                  & 0.522          & 0.389          & 0.381          & 0.323          & 0.234          & 0.177          \\
% $n(\sigma_{X\%})$                            & 0.589          & 0.386          & 0.556          & 0.386          & 0.334          & \textbf{0.247}   \\
% RSD                                           & 0.455          & 0.352          & 0.444          & 0.276          & 0.193          & 0.096          \\
% WAND[$n(\sigma_{X\%})$]                      & 0.566          & 0.386          & \textbf{0.580}  &\textbf{ 0.411}  & 0.236         & 0.142          \\
% NeuralQPP                                    & \textbf{0.611} & \textbf{0.408}  & 0.540          & 0.357          & \textbf{0.367}  & 0.229          \\ \hline
% \multicolumn{7}{|l|}{BERT-Base }                                                                                                                    \\ \hline
% (P@k\_1000)                                & 0.559          & 0.401          & \textbf{0.645}    & \textbf{0.475}  & 0.350          & 0.233          \\
% (AP@1k\_1000)                              & 0.346          & 0.231          & 0.151          & 0.081        & \textbf{0.476}    & \textbf{0.345}          \\
% (P@k\_100)                                 & \textbf{0.585}   & \textbf{0.423}     & 0.637    & 0.454          & 0.393          & 0.271          \\
% (AP@1k\_100)                               & 0.520          & 0.360          & 0.505          & 0.345          & 0.447          & 0.321          \\ \hline
% \multicolumn{7}{|l|}{BERT-Base+Groupwise   }                     \\  \hline
% (Random order\_100)                            & 0.608          & 0.449          & 0.665          & 0.479          & \textbf{0.481} & \textbf{0.353} \\
% (Query order\_100)                             & \textbf{0.615} & 0.456          & 0.676          & 0.486          & 0.455          &  0.327          \\
% (Doc order\_100)                               & 0.563          & 0.383          & 0.660          & 0.476          & 0.365          &  0.262         \\
% (Query+Doc\_100)                               & 0.598          & 0.452          & \textbf{0.682} & \textbf{0.496} & 0.438          &  0.317         \\
% (R+Q+D\_100)                                   & 0.608          & \textbf{0.460} & 0.676          & 0.489          & 0.447          & 0.323          \\ \hline
% \multicolumn{7}{|l|}{BERT-Large+Groupwise}                        \\  \hline
% (BERT\_Large)                            &                &                & 0.645          &  0.461          &                &                \\
% (R+Q+D\_100\_Large)                             & 0.612          & \textbf{0.470} & \textbf{0.688} & \textbf{0.508} & \textbf{0.545} &\textbf{0.399}    \\
% % (Random\_100\_Large)                   &                &                &                &                & 0.531        &  0.396        \\ 
% \hline
% \multicolumn{7}{|l|}{BERT-Small+Groupwise}                        \\ \hline
% (BERT\_Small)                            & 0.591          & 0.391          & 0.615          & 0.436          & 0.394          & 0.278          \\
% (R+Q+D\_100\_Small)                      & 0.590          & 0.419          & 0.680          & 0.500          & 0.437          & 0.305         \\
% % (Random\_100\_Small)                            &                &                &                &                & 0.443          & 0.306          \\ 
% \hline
% \end{tabular} 
% }
% \end{table*}
